Scaling Up and Distilling Down: Language-Guided Robot Skill Acquisition

We present a framework for robot skill acquisition, which 1) efficiently scale up data generation of language-labelled robot data and 2) effectively distills this data down into a robust multi-task language-conditioned visuo-motor policy. For (1), we use a large language model (LLM) to guide high-level planning, and sampling-based robot planners (e.g. motion or grasp samplers) for generating diverse and rich manipulation trajectories. To robustify this data-collection process, the LLM also infers a code-snippet for the success condition of each task, simultaneously enabling the data-collection process to detect failure and retry as well as the automatic labeling of trajectories with success/failure. For (2), we extend the diffusion policy single-task behavior-cloning approach to multi-task settings with language conditioning. Finally, we propose a new multi-task benchmark with 18 tasks across five domains to test long-horizon behavior, common-sense reasoning, tool-use, and intuitive physics. We find that our distilled policy successfully learned the robust retrying behavior in its data collection procedure, while improving absolute success rates by 33.2% on average across five domains. Code, data, and additional qualitative results are available on https://www.cs.columbia.edu/~huy/scalingup/.

==> code_preamble.tex <==

\definecolor{light-gray}{rgb}{0.8, 0.8, 0.8}
\definecolor{comment-green}{rgb}{0.435, 0.576, 0.106}
\definecolor{prompt-blue}{HTML}{2596be}
\definecolor{code-function}{HTML}{379fbe}
\definecolor{code-function}{HTML}{693da8}  %
\definecolor{code-syntax}{HTML}{0060b1}
\definecolor{code-constant}{HTML}{d86001}
\definecolor{prompt-gray}{HTML}{a7a7a7}
\definecolor{highlight}{HTML}{f8f9cb}
\definecolor{highlight}{HTML}{e3eeff}  %
\definecolor{code-perception}{HTML}{2ecc71}
\definecolor{code-control}{HTML}{ff9900}
\definecolor{code-undefined}{HTML}{ff0000}
\renewcommand\fbox{\fcolorbox{light-gray}{white}}

\setlength{\fboxsep}{1.1pt} %
\newcommand{\hlcode}[1]{\colorbox{highlight}{#1}}
\newcommand{\hlcoderesp}[1]{\colorbox{highlight}{\makebox[0.96\linewidth][l]{#1}}}
\newcommand{\link}[1]{\textcolor{magenta}{\href{#1}{#1}}}

\NewDocumentCommand{\code}{v}{%
    \texttt{\small{\textcolor{code-syntax}{#1}}}%
}

\newcommand{\query}[1]{\textcolor{comment-green}{#1}}
\newcommand{\prompt}[1]{\textcolor{prompt-gray}{#1}}
\newcommand{\resp}[1]{#1}

\begingroup\lccode`~=`\_ \lowercase{\endgroup\let~}\_
\catcode`\_=12

==> preamble.tex <==

\usepackage{multicol}
\usepackage{wrapfig}
\usepackage{times}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{siunitx}
\usepackage{gensymb}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{authblk}
\usepackage{pifont}
\usepackage{soul}
\usepackage[symbol]{footmisc}
\usepackage{todonotes}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage{adjustbox}
\usepackage{pdflscape}
\usepackage{bbm}
\usepackage{hyperref}
\usepackage{soul}
\usepackage{listings} %

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\lstset
{ %
   basicstyle=\ttfamily\scriptsize,
   numbers=left,
   stepnumber=1,
   showstringspaces=false,
   tabsize=1,
   breaklines=true,
   breakatwhitespace=false,
   backgroundcolor=\color{backcolour},
   commentstyle=\color{codegreen},
   keywordstyle=\color{magenta},
   numberstyle=\tiny\color{codegray},
   stringstyle=\color{codepurple},
}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\hypersetup{
   colorlinks=true,
   linkcolor=blue,
   urlcolor=blue,
}
\urlstyle{same}
\setcounter{Maxaffil}{0}
\renewcommand\Affilfont{\itshape\small}
\usepackage[moderate]{savetrees}
\usepackage{enumitem}
\setlist[itemize]{leftmargin=2em}
\setlist[enumerate]{leftmargin=2em}

\definecolor{mygreen}{rgb}{0, 0.5, 0}
\definecolor{mygrey}{rgb}{0.6, 0.6, 0.6}
\newcommand{\task}[1]{\textbf{\footnotesize{\texttt{#1}}}}
\newcommand{\cmark}{\textcolor{green}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}%
\newenvironment{myquote}%
{\list{}{\leftmargin=0.3in\rightmargin=0.3in}\item[]}%
{\endlist}

\newcommand{\multitaskbc}{\cite{shridhar2021cliport,shridhar2022peract,zeng2021transporter,jang22a,lynch20a}}
\newcommand{\deepakintrinsic}{\cite{pathak2017curiosity,mendonca2023alan}}

\newcommand{\mypara}[1]{\paragraph{#1}}
\newcommand{\mysection}[1]{\vspace{-3mm}\section{#1}\vspace{-3mm}}
\newcommand{\mysubsection}[1]{\vspace{-3mm}\subsection{#1}\vspace{-3mm}}
\newcommand{\mysubsubsection}[1]{\vspace{-3mm}\subsubsection{#1}\vspace{-3mm}}
\newcommand{\etal}{\textit{et al}. }
\newcommand{\ie}{\textit{i}.\textit{e}., }
\newcommand{\eg}{\textit{e}.\textit{g}. }

\newcommand{\shuran}[1]{\textcolor{blue}{[SS: #1]}}
\newcommand{\huy}[1]{\textcolor{green}{[HH: #1]}}
\newcommand{\pete}[1]{{\color{cyan}\textbf{PF: }#1}\normalfont}
\newcommand{\missing}[1]{\textcolor{red}{#1}}
\newcommand{\notes}[1]{\textcolor{gray}{#1}}

\newcommand{\traj}{\tau}
\newcommand{\success}{s}
\newcommand\inferred[1]{\hat{#1}}
\newcommand\onehot[1]{\mathbbm{1}[{#1}]}
\newcommand{\obs}{o}
\newcommand{\action}{a}
\newcommand{\taskdesc}{\mathcal{T}}

\DeclareMathOperator{\E}{\mathbb{E}}

\definecolor{mygreen}{rgb}{0.78, 1.0, 0.816}
\definecolor{mygreen2}{rgb}{0.235,0.706,0.294}
\definecolor{myred}{rgb}{0.902,0.098,0.294}
\definecolor{myblue}{rgb}{0.263, 0.388, 0.847}

\definecolor{plt_red}{rgb}{0.8588,0.1568,0.1568}
\definecolor{plt_green}{rgb}{0.1725,0.6724,0.1725}
\definecolor{plt_purple}{rgb}{0.34901960784,0.29411764705,0.56862745098}

\DeclareRobustCommand{\hlgreen}[1]{{\sethlcolor{mygreen}\hl{#1}}}

\input{code_preamble}


==> tables/llm_planning_full.tex <==

\begin{table}[t]
    {
        \vspace{-4mm}
        \centering{
            \begin{tabular}{lrrrrrrr}
                \toprule
                Model  & Size & Balance & Catapult & Transport & Mailbox & Drawer & Avg. \\
                \midrule
                LLAMA2 & 7B   & 100     & 0        & 100       & 10      & 0      & 42   \\
                       & 13B  & 100     & 0        & 100       & 90      & 20     & 62
                \\
                \midrule
                GPT3   & 175B & 100     & 90       & 80        & 40      & 100    & 82
                \\
                \midrule
            \end{tabular}
            \caption{
                \textbf{Planning Language Model Evaluation}.
                10 samples per task with temperature 0.1.}
            \label{tab:llm_planning_full}
        }
    }

\end{table}

















==> tables/llm_success_full.tex <==

\begin{table}[t]
    {
        \vspace{-4mm}
        \centering{
            \scriptsize
            \begin{tabular}{lrrrrrrrrr}
                \toprule
                \multirow{2}{*}{ Model} & \multirow{2}{*}{ Size} & \multirow{2}{*}{Balance} & \multicolumn{3}{c}{Catapult} & \multirow{2}{*}{Transport} & \multirow{2}{*}{Mailbox}           \\\cmidrule(lr){4-6}
                                        &                        &                          & Close                        & Mid                        & Far                      &     &   \\
                \midrule
                LLAMA2                  & 7B                     & 80                       & 0                            & 0                          & 0                        & 100 & 0 \\
                                        & 13B                    & 50                       & 0                            & 0                          & 0                        & 100 & 0
                \\
                \midrule
                GPT3                    & 175B                   & 100                      & 100                          & 100                        & 40                       & 100 & 0
                \\
                \midrule
            \end{tabular}

            \begin{tabular}{lrrrrrrrrrrrrrr}
                \toprule
                \multirow{3}{*}{ Model} & \multirow{3}{*}{ Size} & \multicolumn{12}{c}{Drawer} & \multirow{3}{*}{ Avg. (\%)}                                                                                                                      \\
                                        &                        & \multicolumn{3}{c}{Horse}   & \multicolumn{3}{c}{Vitamin} & \multicolumn{3}{c}{Pencilcase} & \multicolumn{3}{c}{Crayon}                                                        \\\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
                                        &                        & T                           & M                           & B                              & T                          & M   & B   & T   & M   & B   & T   & M   & B          \\
                \midrule
                LLAMA2                  & 7B                     & 0                           & 0                           & 0                              & 0                          & 0   & 0   & 0   & 0   & 0   & 0   & 0   & 0   & 10.0 \\
                                        & 13B                    & 100                         & 90                          & 100                            & 60                         & 40  & 20  & 100 & 100 & 100 & 0   & 10  & 0   & 48.3
                \\
                \midrule
                GPT3                    & 175B                   & 100                         & 100                         & 100                            & 100                        & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 91.1
                \\
                \midrule
            \end{tabular}
            \caption{
                \textbf{Success Inference Language Model Evaluation}.
                10 samples per task with temperature 0.1.
                T, M, B stands for top, middle, and bottom respectively.
            }
            \label{tab:llm_success_full}
        }
    }
\end{table}



